HyperBrowseComp: A Multilingual and Multimodal Stress Test for Web-Browsing Agents

We introduce HyperBrowseComp, a multilingual and multimodal browsing benchmark comprising 423 manually authored and human-validated questions across 13 languages, written by native or highly proficient speakers. Questions are designed to be extremely challenging. Each question targets a concise, publicly verifiable answer whose discovery requires locating obscure evidence, following multi-step clue chains, or inspecting heterogeneous sources such as videos, scanned documents, images, or maps. Easier questions are filtered out by evaluating them with models without internet access to reduce the likelihood that they can be answered with parametric knowledge alone. We evaluate several models using provider-native search and a shared external retrieval harness under a common agent protocol. To contextualize model performance and effort, we also conduct a human evaluation on a sample of the questions. HyperBrowseComp provides a challenging testbed for persistent information seeking across languages and evidence modalities, with difficulty arising from discovering and connecting evidence on the open web.

==> figures/effort-analysis.tex <==
% ============================================================
% Native PGFPlots figure. No external image or CSV is needed.
% Required in the main document preamble:
%   \usepackage{xcolor}
%   \usepackage{pgfplots}
%   \usepackage{pgfplotstable}
%   \pgfplotsset{compat=1.18}
% Source: result/model_performance_statistics.json, filtered by
% logs/no-internet-result/retained_ids.txt (417 questions).
% Generated by scripts/export_latex_figures.py; later manual edits
% to these tables will be overwritten if the exporter is rerun.
% ============================================================
\begingroup
\definecolor{hbcPlotBlue}{HTML}{5B7F97}
\definecolor{hbcPlotGreen}{HTML}{789882}
\definecolor{hbcPlotText}{HTML}{18222B}
\definecolor{hbcPlotMuted}{HTML}{78848C}
\definecolor{hbcPlotGrid}{HTML}{E3E8EB}

% ============================================================
% RESULTS -- EDIT THIS BLOCK
% y: 5=Gemini Flash, 4=Gemini Pro, 3=GPT Sol, 2=GPT Terra,
%    1=GPT Luna, 0=Qwen Max (August 19, 2026).
% Only observed runs appear; omitted Exa runs are not zero scores.
% ============================================================
% tokens: THOUSANDS per retained sample with recorded usage, including grading.
% turns: mean agent turns. minutes: mean sample execution time.
\pgfplotstableread[row sep=\\]{
y tokens turns minutes\\
5 33.8228177458 6.1774580336 18.6161745803\\
4 24.301235012 1.2374100719 6.4536725819\\
3 103.1377026379 1.0287769784 2.8347547162\\
2 78.2251534772 1.0551558753 1.5736035971\\
1 65.1475611511 1 1.2031639488\\
0 111.0889434889 11.035971223 7.2612484412\\
}\hbcBuiltin
\pgfplotstableread[row sep=\\]{
y tokens turns minutes\\
4 1332.1269952038 16.8153477218 7.3097342126\\
3 2209.0195251799 14.4556354916 10.6854619504\\
}\hbcExa

% ============================================================
% SHARED APPEARANCE
% ============================================================
\pgfplotsset{
  hbc axis/.style={
    scale only axis,
    ymin=-0.6, ymax=5.6,
    ytick={0,1,2,3,4,5},
    yticklabels={{Qwen 3.8 Max},
      {GPT 5.6 Luna},{GPT 5.6 Terra},{GPT 5.6 Sol},
      {Gemini 3.1 Pro},{Gemini 3.7 Flash}},
    tick style={draw=none},
    ticklabel style={font=\sffamily\scriptsize,text=hbcPlotMuted},
    yticklabel style={font=\sffamily\scriptsize,text=hbcPlotText},
    axis y line*=left, y axis line style={draw=none},
    axis x line*=bottom,
    axis line style={draw=hbcPlotGrid,line width=0.4pt},
    xmajorgrids=true,
    grid style={draw=hbcPlotGrid,line width=0.35pt},
    xlabel style={font=\sffamily\scriptsize,text=hbcPlotMuted},
    title style={font=\sffamily\small,text=hbcPlotText},
    legend style={draw=none,fill=none,font=\sffamily\scriptsize,
      text=hbcPlotText,/tikz/every even column/.append style={column sep=12pt}},
    point meta=x,
    clip=false,
  },
}

\pgfplotsset{
  hbc connector/.style={no marks,draw=hbcPlotMuted!55,
    line width=0.75pt,forget plot},
  hbc builtin/.style={only marks,mark=*,mark size=2.7pt,
    color=hbcPlotBlue},
  hbc exa/.style={only marks,mark=diamond*,mark size=3.1pt,
    color=hbcPlotGreen},
}
% Usage: \input{figures/effort-analysis}
\begin{figure}[!htbp]
\centering
\begin{tikzpicture}
% LEFT: TOKENS (logarithmic axis)
\begin{axis}[
  hbc axis,at={(0,0)},anchor=south west,
  width=0.235\linewidth,height=5.8cm,
  xmode=log,xmin=8,xmax=3500,
  xtick={10,100,1000},xticklabels={10k,100k,1M},
  minor x tick num=0,
  title={(a) Recorded tokens},xlabel={Mean per question (log scale)},
  ymajorgrids=true,
]
\addplot[hbc connector] coordinates {(24.3012350120,4) (1332.1269952038,4)};
\addplot[hbc connector] coordinates {(103.1377026379,3) (2209.0195251799,3)};
\addplot[hbc builtin] table[x=tokens,y=y,meta=tokens]{\hbcBuiltin};
\addplot[hbc exa] table[x=tokens,y=y,meta=tokens]{\hbcExa};
\end{axis}
% CENTER: RECORDED AGENT TURNS
\begin{axis}[
  hbc axis,at={(0.34\linewidth,0)},anchor=south west,
  width=0.235\linewidth,height=5.8cm,
  yticklabels=\empty,
  xmin=-0.6,xmax=20,xtick={0,5,10,15,20},
  title={(b) Agent turns},xlabel={Mean per question},
  ymajorgrids=true,
  legend style={at={(0.5,1.17)},anchor=south,legend columns=2},
]
\addplot[hbc connector] coordinates {(1.2374100719,4) (16.8153477218,4)};
\addplot[hbc connector] coordinates {(1.0287769784,3) (14.4556354916,3)};
\addplot[hbc builtin] table[x=turns,y=y]{\hbcBuiltin};
\addlegendentry{Built-in search}
\addplot[hbc exa] table[x=turns,y=y]{\hbcExa};
\addlegendentry{Exa}
\end{axis}
% RIGHT: SAMPLE EXECUTION TIME
\begin{axis}[
  hbc axis,at={(0.68\linewidth,0)},anchor=south west,
  width=0.235\linewidth,height=5.8cm,
  yticklabels=\empty,
  xmin=-0.6,xmax=21,xtick={0,5,10,15,20},
  title={(c) Execution time},xlabel={Mean minutes per question},
  ymajorgrids=true,
]
\addplot[hbc connector] coordinates {(6.4536725819,4) (7.3097342126,4)};
\addplot[hbc connector] coordinates {(2.8347547162,3) (10.6854619504,3)};
\addplot[hbc builtin] table[x=minutes,y=y]{\hbcBuiltin};
\addplot[hbc exa] table[x=minutes,y=y]{\hbcExa};
\end{axis}
\end{tikzpicture}
\caption{Recorded effort for eight selected runs, grouped by model.
The selected Qwen run is shown.
Circles indicate built-in search and diamonds indicate Exa.
Thin lines connect the two retrieval settings for models evaluated with both.
Panel (a) shows mean recorded tokens per retained sample, including grading,
on a logarithmic axis (k: thousands; M: millions); panel (b) shows mean
recorded agent turns; and panel (c) shows mean sample execution time in
minutes. Points are arithmetic means; sample-time distributions are
right-skewed, so medians and 90th percentiles are reported in the text.
Provider-internal search operations are not necessarily visible
as separate agent turns, and token accounting conventions may differ
across providers. Model names are abbreviated as in Figure~\ref{fig:model-performance}.}
\label{fig:effort-analysis}
\end{figure}
\endgroup


==> figures/language-performance.tex <==
% Native TikZ: \input{figures/language-performance}
% Requires xcolor and tikz (also loaded by pgfplots).
% Generated from result/language_results.csv; exact 417 retained IDs;
% selected Qwen run only.
\begingroup
\definecolor{hbcLangBlue}{HTML}{315B78}
\definecolor{hbcLangInk}{HTML}{18222B}
\definecolor{hbcLangMuted}{HTML}{78848C}
% RESULTS: row / column / correct / scored. Row 12 is the top row.
\def\hbcLanguageCells{
12/0/15/32,
12/1/17/32,
12/2/8/32,
12/3/10/32,
12/4/10/32,
12/5/0/30,
12/6/12/32,
12/7/7/32,
11/0/3/37,
11/1/5/37,
11/2/1/37,
11/3/4/37,
11/4/5/37,
11/5/2/37,
11/6/8/37,
11/7/6/37,
10/0/7/35,
10/1/7/35,
10/2/5/35,
10/3/10/35,
10/4/4/35,
10/5/2/35,
10/6/12/35,
10/7/7/35,
9/0/12/34,
9/1/15/34,
9/2/7/34,
9/3/7/34,
9/4/9/34,
9/5/0/33,
9/6/11/34,
9/7/8/34,
8/0/4/39,
8/1/9/39,
8/2/5/39,
8/3/7/39,
8/4/4/39,
8/5/0/38,
8/6/6/39,
8/7/3/39,
7/0/7/35,
7/1/8/35,
7/2/1/35,
7/3/5/35,
7/4/5/35,
7/5/2/33,
7/6/7/35,
7/7/5/35,
6/0/7/35,
6/1/9/35,
6/2/0/35,
6/3/1/35,
6/4/1/35,
6/5/0/28,
6/6/5/35,
6/7/4/35,
5/0/4/22,
5/1/5/22,
5/2/0/22,
5/3/2/22,
5/4/3/22,
5/5/0/19,
5/6/2/22,
5/7/3/22,
4/0/8/33,
4/1/12/33,
4/2/2/33,
4/3/8/33,
4/4/3/33,
4/5/1/31,
4/6/10/33,
4/7/4/33,
3/0/8/38,
3/1/7/38,
3/2/2/38,
3/3/5/38,
3/4/3/38,
3/5/1/38,
3/6/5/38,
3/7/2/38,
2/0/5/19,
2/1/8/19,
2/2/3/19,
2/3/5/19,
2/4/5/19,
2/5/0/18,
2/6/7/19,
2/7/5/19,
1/0/14/24,
1/1/14/24,
1/2/6/24,
1/3/7/24,
1/4/5/24,
1/5/3/22,
1/6/14/24,
1/7/10/24,
0/0/10/34,
0/1/14/34,
0/2/7/34,
0/3/8/34,
0/4/7/34,
0/5/0/28,
0/6/10/34,
0/7/11/34}
\begin{figure}[!htbp]
\centering
\begin{tikzpicture}[x=0.102\textwidth,y=0.52cm,
 every node/.style={font=\sffamily\scriptsize,text=hbcLangInk,align=center}]
\node[font=\sffamily\small] at (2.5,14) {Built-in search};
\node[font=\sffamily\small] at (6.75,14) {Exa};
\draw[hbcLangMuted!45] (-0.45,13.6)--(5.45,13.6);
\draw[hbcLangMuted!45] (5.8,13.6)--(7.7,13.6);
\node[anchor=east,text=hbcLangMuted] at (-0.65,13) {ID group\\(attempted $n$)};
\node at (0,13) {Gemini\\Pro};
\node at (1,13) {Gemini\\Flash};
\node at (2,13) {GPT\\Luna};
\node at (3,13) {GPT\\Sol};
\node at (4,13) {GPT\\Terra};
\node at (5,13) {Qwen\\Max};
\node at (6.25,13) {GPT\\Sol};
\node at (7.25,13) {Gemini\\Pro};
\node[anchor=east] at (-0.65,12) {ARZ (32)};
\node[anchor=east] at (-0.65,11) {DE (37)};
\node[anchor=east] at (-0.65,10) {ES (35)};
\node[anchor=east] at (-0.65,9) {FIL (34)};
\node[anchor=east] at (-0.65,8) {ID (39)};
\node[anchor=east] at (-0.65,7) {JV (35)};
\node[anchor=east] at (-0.65,6) {KO (35)};
\node[anchor=east] at (-0.65,5) {RU (22)};
\node[anchor=east] at (-0.65,4) {TE (33)};
\node[anchor=east] at (-0.65,3) {TH (38)};
\node[anchor=east] at (-0.65,2) {UZ (19)};
\node[anchor=east] at (-0.65,1) {VI (24)};
\node[anchor=east] at (-0.65,0) {ZH (34)};
\foreach \row/\col/\correct/\scored in \hbcLanguageCells {
 \pgfmathsetmacro{\xx}{\col+ifthenelse(\col>5,0.25,0)}
 \pgfmathsetmacro{\acc}{100*\correct/\scored}
 \fill[hbcLangBlue!\acc!white] (\xx-0.48,\row-0.47) rectangle (\xx+0.48,\row+0.47);
 \ifdim\acc pt>53pt\def\cellInk{white}\else\def\cellInk{hbcLangInk}\fi
 \node[text=\cellInk] at (\xx,\row)
 {\pgfmathprintnumber[fixed,precision=1,fixed zerofill]{\acc}};
}
% Fixed 0--100 scale shared by all configurations.
\foreach \v in {0,...,99} {
 \fill[hbcLangBlue!\v!white] ({2+\v*0.03},-1.3) rectangle ({2+(\v+1)*0.03},-1.02);
}
\node[anchor=east,text=hbcLangMuted] at (1.8,-1.16) {Accuracy (\%)};
\foreach \v/\xx in {0/2,50/3.5,100/5} {
 \node[anchor=north,text=hbcLangMuted] at (\xx,-1.38) {\v};
}
\end{tikzpicture}
\caption{Accuracy by language group inferred from question-ID prefixes.
Cells show the percentage correct among scored questions; row labels give
the number attempted in every run. The eight columns use the same models
and selected runs as Figure~\ref{fig:model-performance}, with only the
selected Qwen3.8-max run. The built-in Qwen run has 27 unscored
attempts that are excluded from its cell denominators;
all other cells have complete scoring. Exact correct/scored counts are
provided in Table~\ref{tab:language-counts}. The groups contain different
questions, so differences do not isolate a causal effect of language.}
\label{fig:language-performance}
\end{figure}
\endgroup


==> figures/model-performance-exa.tex <==
% ============================================================
% Native PGFPlots figure. No external image or CSV is needed.
% Required in the main document preamble:
%   \usepackage{xcolor}
%   \usepackage{pgfplots}
%   \usepackage{pgfplotstable}
%   \pgfplotsset{compat=1.18}
% Source: result/model_performance_statistics.json, filtered by
% logs/no-internet-result/retained_ids.txt (423 questions).
% Generated by scripts/export_latex_figures.py; later manual edits
% to these tables will be overwritten if the exporter is rerun.
% ============================================================
\begingroup
\definecolor{hbcPlotBlue}{HTML}{5B7F97}
\definecolor{hbcPlotGreen}{HTML}{789882}
\definecolor{hbcPlotText}{HTML}{18222B}
\definecolor{hbcPlotMuted}{HTML}{78848C}
\definecolor{hbcPlotGrid}{HTML}{E3E8EB}

% ============================================================
% RESULTS -- EDIT THIS BLOCK
% y: 5=Gemini Flash, 4=Gemini Pro, 3=GPT Sol, 2=GPT Terra,
%    1=GPT Luna, 0=Qwen Max (August 19, 2026).
% Only observed runs appear; omitted Exa runs are not zero scores.
% ============================================================
% Accuracy is a percentage (0--100).
\pgfplotstableread[row sep=\\]{
y accuracy\\
1 25.5319148936\\
0 19.1489361702\\
}\hbcPairedBuiltin
\pgfplotstableread[row sep=\\]{
y accuracy\\
1 18.2033096927\\
0 26.7139479905\\
}\hbcPairedExa

\pgfplotsset{
  hbc paired axis/.style={
    scale only axis,ymin=-0.6,ymax=1.6,ytick={0,1},
    yticklabels={{GPT 5.6 Sol},{Gemini 3.1 Pro}},
    tick style={draw=none},
    ticklabel style={font=\sffamily\scriptsize,text=hbcPlotMuted},
    yticklabel style={font=\sffamily\scriptsize,text=hbcPlotText},
    axis y line*=left,y axis line style={draw=none},axis x line*=bottom,
    axis line style={draw=hbcPlotGrid,line width=0.4pt},xmajorgrids=true,
    grid style={draw=hbcPlotGrid,line width=0.35pt},
    xlabel style={font=\sffamily\scriptsize,text=hbcPlotMuted},
    legend style={draw=none,fill=none,font=\sffamily\scriptsize,
      text=hbcPlotText,/tikz/every even column/.append style={column sep=12pt}},
    point meta=x,clip=false,
  },
}
% Usage: \input{figures/model-performance-exa}
\begin{figure}[!htbp]
\centering
\begin{tikzpicture}
\begin{axis}[
  hbc paired axis,width=0.72\textwidth,height=2.0cm,
  xbar,bar width=6pt,xmin=0,xmax=40,xtick={0,10,20,30,40},
  xlabel={Accuracy (\%)},
  legend style={at={(1,1.14)},anchor=south east},legend columns=2,
  legend image code/.code={\path[#1,draw=none] (0cm,-0.05cm) rectangle (0.20cm,0.05cm);},
  nodes near coords={\pgfmathprintnumber[fixed,precision=1]{\pgfplotspointmeta}\%},
  every node near coord/.append style={font=\sffamily\scriptsize,
    text=hbcPlotText,anchor=west,xshift=2pt},
]
\addplot[xbar,bar shift=3.5pt,fill=hbcPlotBlue,draw=none]
  table[x=accuracy,y=y]{\hbcPairedBuiltin};
\addlegendentry{Built-in search}
\addplot[xbar,bar shift=-3.5pt,fill=hbcPlotGreen,draw=none]
  table[x=accuracy,y=y]{\hbcPairedExa};
\addlegendentry{Exa}
\end{axis}
\end{tikzpicture}
\caption{Within-model comparison of built-in search and Exa. Every run
contains the same 423 retained questions, all of which were scored.}
\label{fig:model-performance-exa}
\end{figure}
\endgroup


==> figures/model-performance.tex <==
% ============================================================
% Native PGFPlots figure. No external image or CSV is needed.
% Required in the main document preamble:
%   \usepackage{xcolor}
%   \usepackage{pgfplots}
%   \usepackage{pgfplotstable}
%   \pgfplotsset{compat=1.18}
% Source: result/model_performance_statistics.json, filtered by
% logs/no-internet-result/retained_ids.txt (423 questions).
% Generated by scripts/export_latex_figures.py; later manual edits
% to these tables will be overwritten if the exporter is rerun.
% ============================================================
\begingroup
\definecolor{hbcPlotBlue}{HTML}{5B7F97}
\definecolor{hbcPlotGreen}{HTML}{789882}
\definecolor{hbcPlotText}{HTML}{18222B}
\definecolor{hbcPlotMuted}{HTML}{78848C}
\definecolor{hbcPlotGrid}{HTML}{E3E8EB}

% ============================================================
% RESULTS -- EDIT THIS BLOCK
% y: 5=Gemini Flash, 4=Gemini Pro, 3=GPT Sol, 2=GPT Terra,
%    1=GPT Luna, 0=Qwen Max (August 19, 2026).
% Only observed runs appear; omitted Exa runs are not zero scores.
% ============================================================
% Accuracy is a percentage (0--100).
\pgfplotstableread[row sep=\\]{
y accuracy\\
5 31.6784869976\\
4 25.5319148936\\
3 19.1489361702\\
2 15.8392434988\\
1 11.5839243499\\
0 2.7848101266\\
}\hbcBuiltin

% ============================================================
% SHARED APPEARANCE
% ============================================================
\pgfplotsset{
  hbc axis/.style={
    scale only axis,
    ymin=-0.6, ymax=5.6,
    ytick={0,1,2,3,4,5},
    yticklabels={{Qwen 3.8 Max},
      {GPT 5.6 Luna},{GPT 5.6 Terra},{GPT 5.6 Sol},
      {Gemini 3.1 Pro},{Gemini 3.7 Flash}},
    tick style={draw=none},
    ticklabel style={font=\sffamily\scriptsize,text=hbcPlotMuted},
    yticklabel style={font=\sffamily\scriptsize,text=hbcPlotText},
    axis y line*=left, y axis line style={draw=none},
    axis x line*=bottom,
    axis line style={draw=hbcPlotGrid,line width=0.4pt},
    xmajorgrids=true,
    grid style={draw=hbcPlotGrid,line width=0.35pt},
    xlabel style={font=\sffamily\scriptsize,text=hbcPlotMuted},
    title style={font=\sffamily\small,text=hbcPlotText},
    legend style={draw=none,fill=none,font=\sffamily\scriptsize,
      text=hbcPlotText,/tikz/every even column/.append style={column sep=12pt}},
    point meta=x,
    clip=false,
  },
}

% Usage: \input{figures/model-performance}
\begin{figure}[!htbp]
\centering
\begin{tikzpicture}
\begin{axis}[
  hbc axis,
  width=0.72\textwidth,height=3.2cm,
  xbar,bar width=5pt,
  xmin=0,xmax=46,xtick={0,10,20,30,40},
  xlabel={Accuracy (\%)},
  nodes near coords={\pgfmathprintnumber[fixed,precision=1]{\pgfplotspointmeta}\%},
  every node near coord/.append style={
    font=\sffamily\scriptsize,text=hbcPlotText,anchor=west,xshift=2pt},
]
\addplot[xbar,bar shift=0pt,fill=hbcPlotBlue,draw=none]
  table[x=accuracy,y=y]{\hbcBuiltin};
\end{axis}
\end{tikzpicture}
\caption{Built-in-search accuracy for the six evaluated models on the same
423 retained questions. Accuracy excludes unscored questions: Qwen
has 395 scored questions, while all other runs have 423.
Shortened model labels refer to the identifiers in the experimental setup.}
\label{fig:model-performance}
\end{figure}
\endgroup


==> figures/question-coverage.tex <==
% Native TikZ diagram. Usage: \input{figures/question-coverage}
% Requires xcolor and tikz (tikz is also loaded by pgfplots).
% Source: result/model_performance_statistics.json and its cited CSV files.
\begingroup
\definecolor{hbcBlue}{HTML}{5B7F97}
\definecolor{hbcGreen}{HTML}{789882}
\definecolor{hbcInk}{HTML}{18222B}
\definecolor{hbcMuted}{HTML}{78848C}
\definecolor{hbcGrid}{HTML}{E3E8EB}

% RESULTS -- EDIT HERE. Categories are disjoint and sum to the total.
\def\hbcTotal{417}
\def\hbcBuiltinCovered{176}
\def\hbcExtraCovered{22}
\def\hbcNeverCorrect{219}
\pgfmathtruncatemacro{\hbcAllCovered}{\hbcBuiltinCovered+\hbcExtraCovered}
\newcommand{\hbcShare}[1]{%
  \pgfmathparse{(#1)/\hbcTotal*100}%
  \pgfmathprintnumber[fixed,precision=1,fixed zerofill]{\pgfmathresult}\%}

\begin{figure}[!htbp]
\centering
\begin{tikzpicture}[
  x=0.32\textwidth,y=1cm,
  every node/.style={font=\sffamily\small,text=hbcInk,align=center},
  hbc card/.style={rounded corners=3pt,text width=0.255\textwidth,
    minimum height=1.55cm,inner sep=8pt,line width=0.6pt},
]
\node[rounded corners=3pt,draw=hbcGrid,fill=hbcGrid!25,
  minimum width=0.29\textwidth,minimum height=0.7cm] (total) at (1,2.05)
  {\textbf{\hbcTotal\ questions}};

\node[hbc card,draw=hbcBlue!65,fill=hbcBlue!9] (builtin) at (0,0)
  {{\large\textbf{\hbcBuiltinCovered}}\ (\hbcShare{\hbcBuiltinCovered})\\[4pt]
   Correct in at least one\\built-in run};
\node[hbc card,draw=hbcGreen!65,fill=hbcGreen!10] (additional) at (1,0)
  {{\large\textbf{\hbcExtraCovered}}\ (\hbcShare{\hbcExtraCovered})\\[4pt]
   Additional questions\\covered by Exa};
\node[hbc card,draw=hbcMuted!45,fill=hbcGrid!35] (uncovered) at (2,0)
  {{\large\textbf{\hbcNeverCorrect}}\ (\hbcShare{\hbcNeverCorrect})\\[4pt]
   No recorded correct\\answer in any run};

\draw[->,hbcMuted,line width=0.6pt] (total.south)--(builtin.north);
\draw[->,hbcMuted,line width=0.6pt] (total.south)--(additional.north);
\draw[->,hbcMuted,line width=0.6pt] (total.south)--(uncovered.north);
\draw[hbcMuted,line width=0.6pt] (-0.42,-1.0)--(-0.42,-1.13)--(1.42,-1.13)--(1.42,-1.0);
\node[anchor=north,font=\sffamily\small] at (0.5,-1.3)
  {\textbf{\hbcAllCovered/\hbcTotal\ (\hbcShare{\hbcAllCovered})}\\[3pt]
   covered across all eight runs};
\end{tikzpicture}
\caption{Retrospective coverage of the 417-question retained evaluation set.
The six selected built-in runs cover 176 questions. The two Exa runs add
22 previously uncovered questions, giving 198 questions with at least one
recorded correct answer across all eight runs. The remaining 219 have no
recorded correct answer; some runs may be unscored on these questions.
These disjoint categories describe observed coverage, not deployable
ensemble accuracy. Qwen uses the selected run only.}
\label{fig:question-coverage}
\end{figure}
\endgroup


==> figures/result_accuracy.tex <==
% ============================================================
% HyperBrowseComp model performance plots
%
% Usage:
%   \input{figures/model-performance}
%
% Required in main preamble:
%   \usepackage{xcolor}
%   \usepackage{pgfplots}
%   \pgfplotsset{compat=1.18}
% ============================================================

\begingroup


% ============================================================
% COLORS
% ============================================================

\definecolor{hbcPlotBlue}{HTML}{5B7F97}
\definecolor{hbcPlotGreen}{HTML}{789882}
\definecolor{hbcPlotText}{HTML}{18222B}
\definecolor{hbcPlotMuted}{HTML}{78848C}
\definecolor{hbcPlotGrid}{HTML}{E3E8EB}


% ============================================================
% RESULTS -- EDIT ONLY THIS BLOCK
% ============================================================
%
% Accuracy: percentage, 0--100
% Tokens: millions
% ============================================================

\def\GeminiProAcc{33.6}
\def\GeminiFlashAcc{37.6}
\def\GPTLunaAcc{15.6}
\def\GPTSolAcc{24.8}
\def\GPTTerraAcc{20.8}
\def\QwenMaxAcc{6.7}

\def\GeminiProTokens{8.0}
\def\GeminiFlashTokens{15.7}
\def\GPTLunaTokens{31.5}
\def\GPTSolTokens{49.5}
\def\GPTTerraTokens{38.0}
\def\QwenMaxTokens{59.0}


% ============================================================
% FIGURE
% ============================================================

\begin{figure*}[t]
\centering

\begin{tikzpicture}


% ============================================================
% LEFT: ACCURACY
% ============================================================

\begin{axis}[
name=accuracyplot,
at={(0,0)},
anchor=south west,
xbar,
width=0.35\textwidth,
height=5.0cm,
scale only axis,
xmin=0,
xmax=100,
ymin=-0.5,
ymax=5.5,
bar width=7pt,
ytick={0,1,2,3,4,5},
yticklabels={
    {Qwen 3.8 Max},
    {GPT 5.6 Terra},
    {GPT 5.6 Sol},
    {GPT 5.6 Luna},
    {Gemini 3.7 Flash},
    {Gemini 3.1 Pro}
},
ytick style={draw=none},
yticklabel style={
    font=\sffamily\scriptsize,
    text=hbcPlotText
},
xtick={0,20,40,60,80,100},
xtick style={draw=none},
xticklabel style={
    font=\sffamily\scriptsize,
    text=hbcPlotMuted
},
axis y line*=left,
y axis line style={draw=none},
axis x line*=bottom,
axis line style={
    draw=hbcPlotMuted,
    line width=0.4pt
},
xmajorgrids=true,
grid style={
    draw=hbcPlotGrid,
    line width=0.35pt
},
xlabel={Accuracy (\%)},
xlabel style={
    font=\sffamily\scriptsize,
    text=hbcPlotMuted
},
nodes near coords={
    \pgfmathprintnumber[
        fixed,
        precision=1
    ]{\pgfplotspointmeta}\%
},
every node near coord/.append style={
    font=\sffamily\bfseries\scriptsize,
    text=hbcPlotText,
    anchor=west,
    xshift=1.2pt
},
point meta=x,
clip=false
]

\addplot[
    xbar,
    fill=hbcPlotBlue,
    draw=none
]
coordinates {
    (\GeminiProAcc,5)
    (\GeminiFlashAcc,4)
    (\GPTLunaAcc,3)
    (\GPTSolAcc,2)
    (\GPTTerraAcc,1)
    (\QwenMaxAcc,0)
};

\end{axis}


% ============================================================
% RIGHT: TOTAL TOKEN USAGE
%
% This value controls the gap between the two plots.
% Tested at 0.43\textwidth.
% ============================================================

\begin{axis}[
at={(0.43\textwidth,0)},
anchor=south west,
xbar,
width=0.35\textwidth,
height=5.0cm,
scale only axis,
xmin=0,
xmax=65,
ymin=-0.5,
ymax=5.5,
bar width=7pt,
ytick={0,1,2,3,4,5},
yticklabels=\empty,
ytick style={draw=none},
xtick={0,10,20,30,40,50,60},
xtick style={draw=none},
xticklabel style={
    font=\sffamily\scriptsize,
    text=hbcPlotMuted
},
axis y line*=left,
y axis line style={draw=none},
axis x line*=bottom,
axis line style={
    draw=hbcPlotMuted,
    line width=0.4pt
},
xmajorgrids=true,
grid style={
    draw=hbcPlotGrid,
    line width=0.35pt
},
xlabel={Total tokens (millions)},
xlabel style={
    font=\sffamily\scriptsize,
    text=hbcPlotMuted
},
nodes near coords={
    \pgfmathprintnumber[
        fixed,
        precision=1
    ]{\pgfplotspointmeta}M
},
every node near coord/.append style={
    font=\sffamily\bfseries\scriptsize,
    text=hbcPlotText,
    anchor=west,
    xshift=1.2pt
},
point meta=x,
clip=false
]

\addplot[
    xbar,
    fill=hbcPlotGreen,
    draw=none
]
coordinates {
    (\GeminiProTokens,5)
    (\GeminiFlashTokens,4)
    (\GPTLunaTokens,3)
    (\GPTSolTokens,2)
    (\GPTTerraTokens,1)
    (\QwenMaxTokens,0)
};

\end{axis}


\end{tikzpicture}

\vspace{-1.5mm}

\caption{
Performance and search cost of evaluated models on \datasetname.
\textbf{Left:} final-answer accuracy.
\textbf{Right:} total token usage across the evaluation set.
}
\label{fig:model-performance}

\end{figure*}

\endgroup

==> figures/retrieval-effects.tex <==
% Native PGFPlots diagram. Usage: \input{figures/retrieval-effects}
% Requires xcolor, pgfplots, and \pgfplotsset{compat=1.18}.
% Source: result/model_performance_statistics.json and its cited CSV files.
\begingroup
\definecolor{hbcBlue}{HTML}{5B7F97}
\definecolor{hbcGreen}{HTML}{789882}
\definecolor{hbcInk}{HTML}{18222B}
\definecolor{hbcMuted}{HTML}{78848C}
\definecolor{hbcGrid}{HTML}{E3E8EB}

% RESULTS -- EDIT HERE. Accuracy differences are percentage points.
\def\hbcSolGain{54}
\def\hbcSolLoss{24}
\def\hbcSolDelta{7.194244604316546}
\def\hbcGemGain{21}
\def\hbcGemLoss{50}
\def\hbcGemDelta{-6.954436450839329}

\pgfplotsset{hbc paired/.style={
  scale only axis,width=0.30\textwidth,height=3.0cm,
  ymin=-0.65,ymax=1.65,ytick={0,1},
  yticklabels={{Gemini 3.1 Pro},{GPT 5.6 Sol}},
  tick style={draw=none},
  ticklabel style={font=\sffamily\scriptsize,text=hbcMuted},
  yticklabel style={font=\sffamily\scriptsize,text=hbcInk},
  axis y line*=left,y axis line style={draw=none},
  axis x line*=bottom,axis line style={draw=hbcGrid},
  xmajorgrids=true,grid style={draw=hbcGrid,line width=0.35pt},
  title style={font=\sffamily\small,text=hbcInk},
  xlabel style={font=\sffamily\scriptsize,text=hbcMuted},
  clip=false,
}}
\begin{figure}[!htbp]
\centering
\begin{tikzpicture}
\begin{axis}[
  hbc paired,at={(0,0)},anchor=south west,
  title={(a) Changed answers},
  xbar,bar width=9pt,xmin=-90,xmax=90,xtick={-80,-40,0,40,80},
  xlabel={Lost $\leftarrow$ Questions $\rightarrow$ Gained},
  point meta=x,
  nodes near coords={\pgfmathprintnumber[fixed,precision=0]{\pgfplotspointmeta}},
]
\draw[hbcMuted,line width=0.5pt] (axis cs:0,-0.65)--(axis cs:0,1.65);
\addplot[xbar,bar shift=0pt,fill=hbcBlue,draw=none,
  every node near coord/.append style={font=\sffamily\scriptsize,
    text=hbcInk,anchor=east,xshift=-2pt}]
  coordinates {(-\hbcSolLoss,1) (-\hbcGemLoss,0)};
\addplot[xbar,bar shift=0pt,fill=hbcGreen,draw=none,
  every node near coord/.append style={font=\sffamily\scriptsize,
    text=hbcInk,anchor=west,xshift=2pt}]
  coordinates {(\hbcSolGain,1) (\hbcGemGain,0)};
\end{axis}

\begin{axis}[
  hbc paired,at={(0.43\textwidth,0)},anchor=south west,
  title={(b) Paired accuracy change},
  xmin=-15,xmax=15,xtick={-15,-10,-5,0,5,10,15},
  yticklabels=\empty,
  xlabel={Exa $-$ built-in (percentage points)},
  point meta=x,
  nodes near coords={\pgfmathprintnumber[fixed,precision=2]{\pgfplotspointmeta}},
  every node near coord/.append style={font=\sffamily\scriptsize,
    text=hbcInk,anchor=south,yshift=6pt},
]
\draw[hbcMuted,dashed,line width=0.5pt] (axis cs:0,-0.65)--(axis cs:0,1.65);
\addplot[only marks,mark=*,mark size=2pt,color=hbcInk]
  coordinates {
    (\hbcSolDelta,1)
    (\hbcGemDelta,0)
  };
\end{axis}
\end{tikzpicture}
\caption{How Exa changes correctness on jointly scored questions.
\textbf{(a)} Blue bars count answers correct only with built-in search
(lost with Exa); green bars count answers correct only with Exa (gained).
\textbf{(b)} Points give the observed matched accuracy difference.
sBoth models use all 417 retained questions.}
\label{fig:retrieval-effects}
\end{figure}
\endgroup


==> result/language_performance_section.tex <==
% Required in the main preamble: \usepackage{placeins}, plus the plot packages.
We stratify the same 417 retained questions into 13 groups using the prefix
of each question ID (Figure~\ref{fig:language-performance};
Table~\ref{tab:language-counts}). We preserve the dataset's prefix codes and
interpret them as language groups; the exported language field is not used
because it contains the loader default \texttt{en} for every selected sample.
Group sizes range from 19 questions for \texttt{UZ} to 39 for \texttt{ID}.
Within each group, accuracy is calculated only over scored questions, with
exact correct/scored counts reported to expose Qwen's incomplete scoring.

\input{figures/language-performance}

Performance varies substantially across groups. The \texttt{VI} group has
the highest observed accuracy for both Gemini built-in configurations:
Gemini 3.7 Flash and Gemini 3.1 Pro Preview each achieve 58.3\% (14/24).
Their lowest observed accuracies are on \texttt{DE}: 13.5\% (5/37) for
Gemini 3.7 Flash and 8.1\% (3/37) for Gemini 3.1 Pro Preview. Giving each
group equal weight yields macro-averaged accuracies of 32.43\% and 26.01\%,
respectively, compared with pooled accuracies of 31.18\% and 24.94\%.
The ordering of the six built-in configurations is unchanged under this
alternative weighting.

The aggregate retrieval effects extend across multiple groups. On questions
scored in both settings, GPT-5.6 Sol improves with Exa in 10 of 13 groups, is
unchanged in two, and declines in one. Its largest gain is on \texttt{VI},
from 29.2\% (7/24) to 58.3\% (14/24), or 29.2 percentage points. Gemini 3.1
Pro Preview declines in nine groups, improves in two, and is unchanged in
two. These comparisons are descriptive: the groups contain different
questions and only 19--39 attempts each, so question difficulty, source
availability, and language are not separately controlled. They should not be
interpreted as causal effects of language or as statistically established
language-specific rankings.

\input{result/language_results_table}
\FloatBarrier


==> result/language_results_table.tex <==
% Exact counts; suitable for an appendix. Requires no extra packages.
\begin{table*}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{5pt}
\begin{tabular}{lrrrrrrrrr}
\hline
& & \multicolumn{6}{c}{Built-in search} & \multicolumn{2}{c}{Exa} \\
ID group & $n$ & G. Pro & G. Flash & GPT Luna & GPT Sol & GPT Terra & Qwen Max & GPT Sol & G. Pro \\
\hline
ARZ & 41 & 22/41 & 25/41 & 11/41 & 16/41 & 15/41 & 3/38 & 19/41 & 15/41 \\
DE & 41 & 6/41 & 8/41 & 3/41 & 5/41 & 7/41 & 2/40 & 11/41 & 7/41 \\
ES & 41 & 11/41 & 9/41 & 8/41 & 12/41 & 5/41 & 3/41 & 14/41 & 11/41 \\
FIL & 41 & 17/41 & 20/41 & 9/41 & 11/41 & 11/41 & 1/39 & 15/41 & 11/41 \\
ID & 41 & 5/41 & 11/41 & 6/41 & 8/41 & 5/41 & 0/40 & 7/41 & 4/41 \\
JV & 41 & 10/41 & 11/41 & 3/41 & 8/41 & 9/41 & 5/39 & 11/41 & 8/41 \\
KO & 41 & 10/38 & 10/41 & 1/41 & 2/41 & 1/41 & 1/31 & 8/41 & 8/41 \\
RU & 31 & 13/30 & 13/31 & 0/31 & 9/31 & 7/31 & 2/28 & 9/31 & 9/31 \\
TE & 41 & 14/40 & 16/41 & 3/41 & 11/41 & 5/41 & 2/36 & 14/41 & 8/41 \\
TH & 40 & 10/39 & 9/40 & 2/40 & 5/40 & 4/40 & 1/40 & 6/40 & 3/40 \\
UZ & 21 & 6/21 & 9/21 & 5/21 & 6/21 & 6/21 & 0/20 & 8/21 & 6/21 \\
VI & 39 & 25/39 & 28/39 & 16/39 & 18/39 & 17/39 & 7/35 & 28/39 & 23/39 \\
ZH & 41 & 17/41 & 19/41 & 11/41 & 13/41 & 12/41 & 4/34 & 17/41 & 15/41 \\
\hline
\end{tabular}
\caption{Exact correct/scored counts by question-ID language group.
$n$ denotes attempted questions per run. Model abbreviations and run
selection follow Figure~\ref{fig:model-performance}. Unscored attempts are
excluded from denominators; no run is pooled with another.}
\label{tab:language-counts}
\end{table*}


==> result/model_performance_section.tex <==
\subsection{Model Performance}
\label{sec:model-performance}

We compare eight evaluation runs spanning six models and two retrieval
settings (Figure~\ref{fig:model-performance}). Each run attempts the same
500 questions. We use the latest Qwen3.8-max run in the retained results,
dated August 19, 2026, and include Exa comparisons for the two models with
complete runs in both settings. Our primary metric is accuracy among
successfully scored questions. We additionally report scoring coverage and
accuracy over all attempted questions, treating unscored attempts as
unsuccessful, to distinguish answer correctness from execution reliability.

With built-in search, Gemini-3.7-flash attains the highest observed accuracy,
37.60\% (188/500), followed by Gemini-3.1-pro-preview at 33.60\% (166/494).
Their respective 95\% Wilson confidence intervals are
$[33.46,41.93]\%$ and $[29.58,37.88]\%$. GPT-5.6-sol, GPT-5.6-terra,
and GPT-5.6-luna achieve 24.80\% (124/500), 20.80\% (104/500), and
15.60\% (78/500), respectively. Qwen3.8-max achieves 6.72\% (31/461).
Scoring coverage is 100\% for all selected runs except built-in Gemini Pro
(98.8\%) and Qwen (92.2\%). Counting their six and 39 unscored questions
as unsuccessful attempts gives accuracies of 33.20\% and 6.20\%,
respectively, without changing the ordering of the observed point estimates.
Even the strongest individual run answers fewer than two in five questions
correctly, indicating substantial remaining difficulty under this protocol.

Exa has contrasting effects on the two models evaluated in both settings.
GPT-5.6-sol improves from 24.80\% to 33.40\% (167/500), a gain of
8.60 percentage points. Gemini-3.1-pro-preview decreases from 33.60\%
to 25.60\% (128/500), an 8.00-point decline in the primary metric.
Because Gemini's scoring coverage differs between settings, we also compare
the 494 questions scored in both runs: built-in search answers 166 correctly
and Exa answers 128 correctly, yielding a matched difference of
$-7.69$ percentage points. On the all-attempted denominator, the difference
is $-7.60$ points. The direction of the Gemini result is therefore unchanged
by these denominator choices.

Question-level pairing reveals changes that aggregate accuracy obscures
(Figure~\ref{fig:retrieval-effects}; Table~\ref{tab:retrieval-transitions}). For GPT-5.6-sol, Exa answers
72 questions correctly that built-in search misses, but fails on 29 that
built-in search answers correctly. The net gain of 43 correct answers thus
reflects both improvements and regressions. For Gemini Pro, Exa gains
25 correct answers but loses 63 on the jointly scored questions. Using
100,000 paired bootstrap resamples of these questions, the 95\% percentile
interval for the accuracy difference is $[4.80,12.60]$ percentage points
for GPT-5.6-sol and $[-11.34,-4.05]$ for Gemini Pro. These intervals
preserve the pairing of outcomes for each question and are conditional on
the observed runs and grades; they do not capture variation across repeated
model runs, changes in web content, or grading uncertainty.

The runs also exhibit complementary successes (Figure~\ref{fig:question-coverage}).
Across the six built-in
search runs, at least one model produces a recorded correct answer on
249 of the 500 questions (49.8\%). Including the two Exa runs increases
this coverage to 274 questions (54.8\%), adding 25 questions not answered
correctly by any selected built-in run. Conversely, 226 questions have no
recorded correct answer across all eight runs. This is a retrospective
coverage measure, not an achievable ensemble accuracy: selecting a correct
answer would require an additional selection procedure. Nevertheless, it
shows that the runs' successes are not identical, while a large subset of
questions remains unresolved by every evaluated configuration.

\input{result/language_performance_section}

Performance must also be considered alongside the effort required to obtain
it (Section~\ref{sec:effort-analysis}). GPT-5.6-sol's 8.60-point gain with
Exa accompanies an increase from approximately 99,091 to 2,012,480 recorded
tokens per attempted question ($20.31\times$), from 1.03 to 13.60 mean
agent turns, and from 2.75 to 9.88 minutes of mean sample execution time.
Gemini Pro uses approximately 16,178 tokens per question with built-in
search and 1,253,317 with Exa ($77.47\times$), while mean turns increase
from 1.16 to 16.01 and mean sample time increases from 5.96 to 6.95 minutes,
despite the accuracy decline. Thus, additional recorded effort does not
consistently translate into higher accuracy. Token totals include grading
and run-level overhead, and recorded turns need not expose provider-internal
search operations; these ratios should not be interpreted as equivalent
ratios of monetary cost or reasoning computation.

These results characterize the evaluated model--retrieval configurations
rather than isolating model reasoning ability. Built-in search systems
differ across providers, the two retrieval settings were evaluated at
different times, and each model grades its own responses using a common
grading prompt. Accordingly, the results support a model-dependent effect
of the Exa harness in these runs, rather than a general claim that one
retrieval setting is superior. The retained results contain no no-internet
evaluations, so the planned parameter-only baseline and its associated
question-exclusion analysis remain pending.

\input{figures/model-performance}

\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{6pt}
\begin{tabular}{lrrrrrr}
\hline
Model & Paired $n$ & Both correct & Built-in only & Exa only & Neither & $\Delta$ (pp) \\
\hline
GPT-5.6-sol & 500 & 95 & 29 & 72 & 304 & $+8.60$ \\
Gemini-3.1-pro-preview & 494 & 103 & 63 & 25 & 303 & $-7.69$ \\
\hline
\end{tabular}
\caption{Paired correctness outcomes for questions scored under both
retrieval settings. ``Built-in only'' counts correct answers lost with Exa;
``Exa only'' counts newly correct answers. $\Delta$ is Exa accuracy minus
built-in accuracy on the paired subset, in percentage points. Six Gemini
questions without a built-in score are excluded; all six are incorrect
under Exa.}
\label{tab:retrieval-transitions}
\end{table*}

\input{figures/retrieval-effects}
\input{figures/question-coverage}
\input{figures/language-performance}
\input{result/language_results_table}


==> result/report_sections.tex <==
% Requires xcolor, pgfplots, pgfplotstable and pgfplots compat=1.18.
% Keep the figures/ directory beside your main LaTeX file.

\subsection{Model Performance}
\label{sec:model-performance}

We compare eight evaluation runs spanning six models and two retrieval
settings (Figure~\ref{fig:model-performance}). Each run attempts the same
500 questions. We use the latest Qwen3.8-max run in the retained results,
dated August 19, 2026, and include Exa comparisons for the two models with
complete runs in both settings. Our primary metric is accuracy among
successfully scored questions. We additionally report scoring coverage and
accuracy over all attempted questions, treating unscored attempts as
unsuccessful, to distinguish answer correctness from execution reliability.

With built-in search, Gemini-3.7-flash attains the highest observed accuracy,
37.60\% (188/500), followed by Gemini-3.1-pro-preview at 33.60\% (166/494).
Their respective 95\% Wilson confidence intervals are
$[33.46,41.93]\%$ and $[29.58,37.88]\%$. GPT-5.6-sol, GPT-5.6-terra,
and GPT-5.6-luna achieve 24.80\% (124/500), 20.80\% (104/500), and
15.60\% (78/500), respectively. Qwen3.8-max achieves 6.72\% (31/461).
Scoring coverage is 100\% for all selected runs except built-in Gemini Pro
(98.8\%) and Qwen (92.2\%). Counting their six and 39 unscored questions
as unsuccessful attempts gives accuracies of 33.20\% and 6.20\%,
respectively, without changing the ordering of the observed point estimates.
Even the strongest individual run answers fewer than two in five questions
correctly, indicating substantial remaining difficulty under this protocol.

Exa has contrasting effects on the two models evaluated in both settings.
GPT-5.6-sol improves from 24.80\% to 33.40\% (167/500), a gain of
8.60 percentage points. Gemini-3.1-pro-preview decreases from 33.60\%
to 25.60\% (128/500), an 8.00-point decline in the primary metric.
Because Gemini's scoring coverage differs between settings, we also compare
the 494 questions scored in both runs: built-in search answers 166 correctly
and Exa answers 128 correctly, yielding a matched difference of
$-7.69$ percentage points. On the all-attempted denominator, the difference
is $-7.60$ points. The direction of the Gemini result is therefore unchanged
by these denominator choices.

Question-level pairing reveals changes that aggregate accuracy obscures
(Figure~\ref{fig:retrieval-effects}; Table~\ref{tab:retrieval-transitions}). For GPT-5.6-sol, Exa answers
72 questions correctly that built-in search misses, but fails on 29 that
built-in search answers correctly. The net gain of 43 correct answers thus
reflects both improvements and regressions. For Gemini Pro, Exa gains
25 correct answers but loses 63 on the jointly scored questions. Using
100,000 paired bootstrap resamples of these questions, the 95\% percentile
interval for the accuracy difference is $[4.80,12.60]$ percentage points
for GPT-5.6-sol and $[-11.34,-4.05]$ for Gemini Pro. These intervals
preserve the pairing of outcomes for each question and are conditional on
the observed runs and grades; they do not capture variation across repeated
model runs, changes in web content, or grading uncertainty.

The runs also exhibit complementary successes (Figure~\ref{fig:question-coverage}).
Across the six built-in
search runs, at least one model produces a recorded correct answer on
249 of the 500 questions (49.8\%). Including the two Exa runs increases
this coverage to 274 questions (54.8\%), adding 25 questions not answered
correctly by any selected built-in run. Conversely, 226 questions have no
recorded correct answer across all eight runs. This is a retrospective
coverage measure, not an achievable ensemble accuracy: selecting a correct
answer would require an additional selection procedure. Nevertheless, it
shows that the runs' successes are not identical, while a large subset of
questions remains unresolved by every evaluated configuration.

\input{result/language_performance_section}

Performance must also be considered alongside the effort required to obtain
it (Section~\ref{sec:effort-analysis}). GPT-5.6-sol's 8.60-point gain with
Exa accompanies an increase from approximately 99,091 to 2,012,480 recorded
tokens per attempted question ($20.31\times$), from 1.03 to 13.60 mean
agent turns, and from 2.75 to 9.88 minutes of mean sample execution time.
Gemini Pro uses approximately 16,178 tokens per question with built-in
search and 1,253,317 with Exa ($77.47\times$), while mean turns increase
from 1.16 to 16.01 and mean sample time increases from 5.96 to 6.95 minutes,
despite the accuracy decline. Thus, additional recorded effort does not
consistently translate into higher accuracy. Token totals include grading
and run-level overhead, and recorded turns need not expose provider-internal
search operations; these ratios should not be interpreted as equivalent
ratios of monetary cost or reasoning computation.

These results characterize the evaluated model--retrieval configurations
rather than isolating model reasoning ability. Built-in search systems
differ across providers, the two retrieval settings were evaluated at
different times, and each model grades its own responses using a common
grading prompt. Accordingly, the results support a model-dependent effect
of the Exa harness in these runs, rather than a general claim that one
retrieval setting is superior. The retained results contain no no-internet
evaluations, so the planned parameter-only baseline and its associated
question-exclusion analysis remain pending.

\input{figures/model-performance}

\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{6pt}
\begin{tabular}{lrrrrrr}
\hline
Model & Paired $n$ & Both correct & Built-in only & Exa only & Neither & $\Delta$ (pp) \\
\hline
GPT-5.6-sol & 500 & 95 & 29 & 72 & 304 & $+8.60$ \\
Gemini-3.1-pro-preview & 494 & 103 & 63 & 25 & 303 & $-7.69$ \\
\hline
\end{tabular}
\caption{Paired correctness outcomes for questions scored under both
retrieval settings. ``Built-in only'' counts correct answers lost with Exa;
``Exa only'' counts newly correct answers. $\Delta$ is Exa accuracy minus
built-in accuracy on the paired subset, in percentage points. Six Gemini
questions without a built-in score are excluded; all six are incorrect
under Exa.}
\label{tab:retrieval-transitions}
\end{table*}

\input{figures/retrieval-effects}
\input{figures/question-coverage}
\input{figures/language-performance}
\input{result/language_results_table}

\subsection{Effort Analysis}
\label{sec:effort-analysis}

We characterize effort using recorded tokens per attempted question, mean
agent turns, and mean sample execution time (Figure~\ref{fig:effort-analysis}).
Tokens per question are calculated by dividing the run-level token total by
500, including grading calls and any additional usage recorded at run level.
This differs from averaging only saved samples with available token usage:
some headers contain more tokens than their saved-sample totals. These
measurements describe recorded evaluation effort, not monetary cost or a
uniform measure of computation across providers. Agent turns likewise count
harness-level interactions; a built-in search request may perform additional
provider-side work that is not exposed as separate turns.

Exa substantially increases recorded tokens and turns for both comparable
models. For GPT-5.6-sol, tokens per question rise from approximately 99,091
to 2,012,480, a 20.31-fold increase, while mean turns rise from 1.03 to 13.60.
Mean sample time increases from 2.75 to 9.88 minutes. Its 8.60-percentage-point
accuracy gain therefore accompanies substantially greater recorded effort.
For Gemini-3.1-pro-preview, tokens per question rise from approximately
16,178 to 1,253,317, a 77.47-fold increase, and mean turns rise from 1.16 to
16.01. Mean sample time increases more modestly, from 5.96 to 6.95 minutes,
despite the decrease in accuracy. Increased recorded effort therefore does
not consistently translate into better answers. The token increases should
not be interpreted as proportional increases in reasoning: input and
cache-read tokens together account for 99.77\% of GPT-5.6-sol's Exa token
total and 98.79\% of Gemini-3.1-pro-preview's.

Effort also varies substantially within the built-in search setting.
GPT-5.6-luna has the lowest mean sample time at 1.18 minutes, while
Gemini-3.1-pro-preview has the lowest recorded token total per question at
approximately 16,178. Gemini-3.7-flash combines the highest observed accuracy
with the largest mean sample time, 17.11 minutes, although its median is only
2.40 minutes. This gap indicates a long upper tail in execution times rather
than uniformly slow responses. Qwen3.8-max averages 10.87 turns despite
its low accuracy, further showing that additional turns
alone are not a reliable indicator of successful problem solving. We use
sample execution times rather than whole-run wall times, which also depend
on concurrency and scheduling; sample times can still reflect retries and
service delays.

\input{figures/effort-analysis}

